m-Nearly k-Universal Words -- Investigating Simon Congruence

Determining the index of the Simon congruence is a long outstanding open problem. Two words $u$ and $v$ are called Simon congruent if they have the same set of scattered factors, which are parts of the word in the correct order but not necessarily consecutive, e.g., $\mathtt{oath}$ is a scattered factor of $\mathtt{logarithm}$. Following the idea of scattered factor $k$-universality, we investigate $m$-nearly $k$-universality, i.e., words where $m$ scattered factors of length $k$ are absent, w.r.t. Simon congruence. We present a full characterisation as well as the index of the congruence for $m=1$. For $m\neq 1$, we show some results if in addition $w$ is $(k-1)$-universal as well as some further insights for different $m$.

==> content/proofs/sec-mnearly/proof_iota=k-1.tex <==
\begin{proof}
%	{\color{blue}
%		Suppose $\iota(w)\leq k-2$. Thus, we have $|m(w)|=\iota(w)$ and $\ScatFact_{\iota(w)}(w)=\Sigma^{\iota(w)}$ 
%		as well as 
%		$\ScatFact_{\iota(w)+t}(w)\subset\Sigma^{\iota(w)+t}$ for all $t\in\N$. Moreover we have $r(w)\subset\Sigma$. 
%		This implies that each word $u\in\Sigma^k$ with $u=m(w)v$ and $v\not\in\ScatFact_{k-\iota(w)}(r(w))$ is not a 
%		scattered factor of $w$ of length $k$.
%		\begin{itemize}
%			\item If all letters from $v$ are from $\Sigma\backslash\letters(r(w))$ then we have 
%			$(|\Sigma|-\ell)^{k-\iota(w))}$
%			possibilites for $v$.
%			\item If all letters but one from $v$ are from $\Sigma\backslash\letters(r(w))$, then we have for each of the 
%			positions where the letter from $\letters(r(w))$ occurs $(|\Sigma|-\ell)^{k-\iota(w)-1}$ possibilities and since 
%			we have $k-\iota(w)-1$ positions for the letter from $\letters(r(w))$ we get 
%			$(k-\iota(w))(|\Sigma|-\ell)^{k-\iota(w)-1}$ possibilities; moreover we have $\ell$ options to choose this 
%			letter and thus we have in total $\ell(k-\iota(w)+1)(|\Sigma|-\ell)^{k-\iota(w)-1}$
%			\item In general, if $i$ letters of $v$ are from $\letters(r(w))$, we have
%			\begin{itemize}
%				\item $\binom{k-\iota(w)}{i}$ possibilities to place these $i$ letters, since we have $\ell$ letters in 
%				$r(w)$, we have $\ell^i\binom{k-\iota(w)}{i}$ possibilities for these words
%				\item for the remaining $k-\iota(w)-i$ positions we can use all words over $\Sigma\backslash\letters(r(w))$,
%				these are $(|\Sigma|-\ell)^{k-\iota(w)-i}$ many.
%				\item Thus, we have $\ell^i\binom{k-\iota(w)}{i}(|\Sigma|-\ell)^{k-\iota(w)-i}$ possibilities to choose $v$
%			\end{itemize}
%			\item in total, we get $\sum_{i=0}^{k-\iota(w)-1}\ell^i\binom{k-\iota(w)}{i}(|\Sigma|-\ell)^{k-\iota(w)-i}$    
%			possibilities for $v$
%		\end{itemize}
%		\bigskip
%		
%		
%		
%		
%	}
	Suppose $\iota(w)=k-2$. Thus, we have $|m(w)|=k-2$ and $\ScatFact_{k-2}(w)=\Sigma^{k-2}$ as well as 
	$\ScatFact_{k-1}(w)\subset\Sigma^{k-1}$. Moreover we have $r(w)\subset\Sigma$. 
	This implies immediately that $(|\Sigma|-\ell)^2$ words are not scattered factors of length $2$ of $r(w)$. 
	Moreover
	each word in 
	\[
	M=\letters(r(w))(\Sigma\backslash\letters(r(w)))\cup(\Sigma\backslash\letters(r(w))\letters(r(w))
	\]
	is not in $\ScatFact_2(r(w))$, these are $2\ell(|\Sigma|-\ell)$ many. Since each $m(w)u\not\in\ScatFact_k(w)$ 
	for all $u\in M\cup(\Sigma\backslash\letters(r(w)))^2$, we obtain
	
	\[
	m\geq (|\Sigma|-\ell)^2+2\ell(|\Sigma|-\ell)
	\]
	
	
	\bigskip
	
	\begin{align*}
	|\Sigma|^k - m = |\ScatFact_k(w)|&\leq|\Sigma|^k-(|\Sigma|-\ell)^2-2\ell(|\Sigma|-\ell)\\
	&=|\Sigma|^k-|\Sigma|^2+2|\Sigma|\ell-\ell^2-2\ell|\Sigma|+2\ell^2\\
	&=|\Sigma|^k-|\Sigma|^2+\ell^2.
	\end{align*}
	\begin{align*}
	&\Leftrightarrow |\Sigma|^k -m \leq |\Sigma|^k-|\Sigma|^2+\ell^2\\
	&\Leftrightarrow m \geq |\Sigma|^2 - \ell^2
	\end{align*}
	Thus for all $m<|\Sigma|^2 - \ell^2$ we get a contradiction.
\end{proof}%}

==> content/proofs/sec-mnearly/proof_sorted.tex <==
\begin{proof}
Let $w\in\NUniv_{\Sigma,\sigma^k-2,k}$. By Lemma~\ref{2insidek+1} we have $|\alph(w)|=2$. Suppose there exist $r_1,r_2,r_3\in\N$ and
$w_1\in\Sigma^{\ast}$ with $w=\ta^{r_1}\tb^{r_2}\ta^{r_3}w_1$, i.e., $|\cond(w)|>2$ (we assume w.l.o.g. that $w[1]=\ta$).
Set $u_1=\ta^{s_1-1}\tb^{s_2}\ta^{s_3}v_1$, $u_2=\ta^{s_1}\tb^{s_2-1}\ta^{s_3}v_1$, $u_3=\ta^{s_1}\tb^{s_2}\ta^{s_3-1}v_1$ such that $s_1-1+s_2+s_3+|v_1|=k$
for $s_i\leq r_i$, $i\in[3]$, $v_1\in\Pref(w_1)$. Then $u_1,u_2$, and $u_3$ are different scattered factors of $w$ - a contradiction.\qed
\end{proof}


==> content/proofs/sec-nearly/proof-nearly_with_unary_modus_product.tex <==
\begin{proof}
%	(Induction on $k \in \N$)
%	For $k = 1$ we have only the rest $\varphi(\ta_1 \cdots \ta_{n-1})$ which is nearly $1$-universal by \autoref{fundamental}.
%	Suppose that each word \[w \in (\varphi(\ta_1 \cdots \ta_{n-1})\ta_n)^{k-1} \varphi(\ta_1 \cdots \ta_{n-1})\] is nearly $k$-universal for a $k \in \mathbb{N}$. Now 
	Consider $k \in \N$ and all words \[w \in \left(\prod_{i=1}^{k-1} \varphi_i(\ta_1\dots \ta_{n-1})\ta_n\right) \varphi_k(\ta_1\dots \ta_{n-1}).\] 
	Since there are $k-1$ arches and a rest, $w$ cannot be $k$-universal. Thus, suppose that we have $u \notin \operatorname{ScatFact}_{k}(w)$ with $u \neq \ta_n^{k}$. So there exists an $i \in [k-1]$ with $u[i] \neq \ta_n^{k}[i] = \ta_n$. In the case of $i < k$ we can find the first $i$ letters in the first $i$ arches with $u[i] \neq \ta_n[i]$. If we find an $\tilde{i} \in [k-1]$ with $u[\tilde{i}]u[\tilde{i}+1] \in \operatorname{ScatFact}_2(\operatorname{ar}_{\tilde{i}}(w))$, i.e. $u[\tilde{i}]$ and $u[\tilde{i}+1]$ are in the same arch, then there are $k-1-\tilde{i}$ arches left to find the last $k-(i+1) = k-i-1$ letters of $u$. Thus, $u$ cannot be a missing scattered factor, if we find $u[\tilde{i}]$ and $u[\tilde{i}+1]$ both in the $i^{\text{th}}$ arch. Therefore, we know that $u[i] \in \operatorname{ScatFact}_1(\operatorname{ar}_i(w))$. Since there are $k-1$ arches $w$ contains all scattered factors of length $k-1$. Now those scattered factors of length $k-1$ can be extended to scattered factors of length $k$ by every letter in $\{\ta_1, \dots, \ta_{n-1}\}$. We can conclude that $\ta_n^k$ is the only missing scattered factor.
%	
%	To proof the nearly $k$-universality we need to show that $\abs{\operatorname{ScatFact}_{k}(w)} = \abs{\Sigma}^{k} -1$. We know that $\ta_j^{k} \in \operatorname{ScatFact}_{k}(w)$ for every $j \in [k-1]$. For every combination of length $k-1$ of $\ta_1 \dots \ta_n$ we also know that these combinations are in $w$. Since we can find each letter of $\{\ta_1, \dots, \ta_{n-1}\} $ to put in the end $\ta_n^{k}$ is the only missing scattered factor.
\end{proof}

==> content/proofs/sec-nearly/proof-upperboundk.tex <==
\begin{proof}
	Let $w \in \Sigma^n$ be nearly $k$-universal. Then by Remark~\ref{alph} we have $n\geq k\sigma-1$ and therefore we get $k\leq \frac{n+1}{\sigma}$. For the second direction, let $k\leq\lfloor\frac{n+1}{\sigma}\rfloor$ and $u=\ta^k$ for some $\ta\in\Sigma$. Thus, we have $\cond(u)=1$ and by Theorem~\ref{length} we get $|w_u|=k\sigma+1-2\leq
	\lfloor\frac{n+1}{\sigma}\rfloor\sigma-1\leq n$. Now we apply Lemma~\ref{paperstream} to obtain  $w\in\NUniv_{\Sigma,1,k}\cap\Sigma^n$.\qed
\end{proof}

